Strong convexity-guided hyper-parameter optimization for flatter losses

We propose a novel white-box approach to hyper-parameter optimization. Motivated by recent work establishing a relationship between flat minima and generalization, we first establish a relationship between the strong convexity of the loss and its flatness. Based on this, we seek to find hyper-parameter configurations that improve flatness by minimizing the strong convexity of the loss. By using the structure of the underlying neural network, we derive closed-form equations to approximate the strong convexity parameter, and attempt to find hyper-parameters that minimize it in a randomized fashion. Through experiments on 14 classification datasets, we show that our method achieves strong performance at a fraction of the runtime.

==> conv.tex <==
\subsubsection{Convolutional classifiers}
\label{sec:conv}

This section focuses on convolutional neural networks that use max-pooling, ReLU activations in the intermediate layers, and a flattening layer after all convolutional layers that is fed to a one-layer feedforward network with a softmax activation. We also assume cross-entropy loss. These are standard settings that are used, and thus not strong assumptions. 

For convolutional neural networks, it is difficult to compute a closed-form solution to the strong convexity. Therefore, we choose to compute the maximum \textit{smoothness} instead. As discussed in Section \ref{sec:stcvx:approx:smooth}, the maximum smoothness is a loose upper bound on the strong convexity. We choose to use this looser bound since experimentally, we found that this leads to flat minima (see Figure \ref{fig:smoothness-hpo}), which is known to be useful for generalization.

We assume that the network is comprised of Conv --$>$ ReLU --$>$ MaxPool blocks. The order of the ReLU and MaxPool, as we will later see, is not important. In this discussion, we will not include batch normalization or dropout.

Redefine $L$ to be the number of convolutional blocks, and at layer $l$, the input is convoluted with a kernel $k^{[l]}$, added to a bias vector $b^{[l]}$ (resulting in $z^{[l]}$), followed by a ReLU activation (resulting in $C^{[l]}$), and a max-pooling (resulting in $P^{[l]}$). After all convolutional layers, the output is flattened (resulting in $P^{[L]f}$), and passed to a feedforward network with weights $w$ and biases $b$, followed by a softmax layer.

In the forward propagation step, we perform the following (where $\lambda$ is the pooling parameter:
\begin{align}
    z^{[l]}_{muv} &= \sum\limits_n \sum\limits_n \sum\limits_q P^{[l-1]}_{n, p+u, q+v} k^{[l]}_{mnpq} + b^{[l]}_m \\
    C^{[l]}_{muv} &= \max (0, z^{[l]}_{muv}) \\
    P^{[l]}_{mxy} &= \max C^{[l]}_{muv} \\
    & u = \lambda x, \ldots, (\lambda + 1) x - 1 \\
    & v = \lambda y, \ldots, (\lambda + 1) y - 1
\end{align}

at the feedforward layer, we then do:
$$
S = \sum\limits_{j} w_{j} P^{[L]f} + b
$$

In Theorem \ref{th:conv:smoothness}, we show that the smoothness of the loss function is 
$$
    \beta = \frac{\lVert P^{[L]} \rVert}{\lVert P^{[L]f} \rVert} \lVert w \rVert \lVert z^{[L-1]} \rVert
$$

==> smoothness.tex <==
\subsection{Approximating the strong convexity in mini-batches}
\label{sec:covering}

If the Hessian is well-conditioned, then its norm can be bounded. As such, we can use the standard covering number guarantee (cf. \citet{duchi2023}, Example 4.3.9)

% In this section, we show why it is reasonable to use a mini-batch approach to compute the strong convexity for the loss function. We use an argument similar to \citet{duchi2023}. %, Example 4.3.9.

% Consider a set of random variables $X_i$ and let $f: \mathcal{X} \mapsto \mathbb{R}$ be a function over a separable space $\mathcal{X}$. Let $P_n f = \frac{1}{n} \sum\limits_{i=1}^n f(X_i)$ be the empirical distribution of $f$ and let $P_f = \int f(x) \mathrm{d}P(x)$ be the general expectation under a measure $P$. Denote by $N(\delta, \Theta, \rho)$, the $\delta-$covering number of a set $\Theta$ under a metric $\rho$. In Theorem \ref{th:minibatch-bound}, we prove the following bound:
% \begin{equation}
%     \mathbb{P}\left( \sup\limits_{f \in \mathcal{F}} \abs{P_nf - Pf} \geq t \right) \leq \exp\left( -\frac{2nt^2}{9mb^2} + \log N \right)
% \end{equation}
% where $m = \dim f$ and $\norm{P_n f_i - P_n f}_\infty \leq b$ for the covering functions $f_i$.

% \subsection{Smoothness as an approximation for strong convexity}
% \label{sec:stcvx:approx:smooth}

% In some cases such as convolutional networks, it is tricky to compute a \textit{lower bound} on the norm of the Hessian. However, it is easier to compute an \textit{upper bound}. This yields the $\beta-$smoothness of the loss. We can use the $\beta-$smoothness to approximate the strong convexity. To see why, consider the max-min inequality:
% $$
% \sup\limits_x \inf\limits_y f(x, y) \leq \inf\limits_x \sup\limits_y f(x, y)
% $$

% We extend this as follows:

% \begin{equation}
%     \sup\limits_x \inf\limits_y f(x, y) \leq \inf\limits_x \sup\limits_y f(x, y) \leq \sup\limits_x \sup\limits_y f(x, y) \label{eq:maxmin}
% \end{equation}

% Set $f(\cdot) = \lVert \nabla^2 \mathcal{L} \rVert$ for a loss function $\mathcal{L}$, and parameterize the loss as $\mathcal{L}(X, h)$ (i.e., the loss depends on the data and the hyper-parameters chosen). Next, rewrite the above equation as follows:

% \begin{equation}
%     \sup\limits_h \inf\limits_X f(X, h) \leq \inf\limits_h \sup\limits_X f(X, h) \leq \sup\limits_h \sup\limits_X f(X, h) \label{eq:maxmin:2}
% \end{equation}

% so that $\sup\limits_X f(X, h) = \beta$, the $\beta-$smoothness. The middle term, which searches for a minima of the smoothness, is suggested by convex optimization literature. Instead, we compute the right-most part of \eqref{eq:maxmin:2}. Next, observe that the left-most part of \eqref{eq:maxmin:2} is the \textit{strong convexity parameter} $\mu$.

% It is well-known that the higher the strong convexity parameter, the more well-behaved the function is. Therefore, as \eqref{eq:maxmin:2} describes, it is in our interest to maximize this value. However, computing the minimum norm of the Hessian is trickier than computing the maximum (which the other two parts of the equation use), so we instead accept a looser upper bound on the strong convexity parameter instead. Therefore, using configurations with high $\beta-$smoothness values is equivalent to choosing configurations with a loose upper bound on their strong convexity parameter.

% \subsubsection{Why maximize smoothness?}

% \begin{figure}[t]
%     \centering
%     \includesvg[width=.5\textwidth]{img/post.svg}
%     \caption{Flat minima observed when using maximum smoothness as a heuristic for HPO.}
%     \label{fig:smoothness-hpo}
% \end{figure}

% Astute readers of the above discussion likely noticed that we choose to \textit{maximize} the $\beta-$smoothness, while traditional convex optimization literature motivates minimizing it. Here, we will motivate this with two different reasons.

% \begin{enumerate}
%     \item \textit{The maximum smoothness is a loose approximation of the maximum strong convexity.}
%     Here, it is important to quantify how loose this approximation is. Precisely, we seek
%     \begin{equation}
%         \sup \abs{
%             \sup\limits_h \sup\limits_X \norm{\nabla^2 \mathcal{L}} - \sup\limits_h \inf\limits_X \norm{\nabla^2 \mathcal{L}}
%         }
%         \label{eq:smoothness:bounds}
%     \end{equation}
%     We can now proceed to quantify this.
%     \begin{lemma}[Looseness of smoothness approximation]
%         Suppose $\nabla^2 \mathcal{L}$ is $M-$Lipschitz continuous. For $x, y \in \mathbb{R}^d$, let $\norm{x - y} 
%         \leq r$. Then
%         \eqref{eq:smoothness:bounds} is $Mr$.
%     \end{lemma}
%     \begin{proof}
%         From \eqref{eq:smoothness:bounds},
%         \begin{align*}
%             &\sup \abs{
%                 \sup\limits_h \sup\limits_X \norm{\nabla^2 \mathcal{L}} - \sup\limits_h \inf\limits_X \norm{\nabla^2 \mathcal{L}}
%             } \\
%             &\leq \sup\limits_h \abs{
%             \sup\limits_X \norm{\nabla^2 \mathcal{L}} - \inf\limits_X \norm{\nabla^2 \mathcal{L}}
%         } \\
%         &= \sup\limits_h \abs{\beta_h - \mu_h} \\
%         &\leq \beta_{max} - \mu_{min}
%         \end{align*}

%         where $\beta_{max} = \sup\limits_h \sup\limits_X \norm{\nabla^2 \mathcal{L}}$ and $\mu_{min} = \inf\limits_h \inf\limits_X \norm{\nabla^2 \mathcal{L}}$.

%         From Lipschitz continuity, 
%         $$
%         \norm{\nabla^2 \mathcal{L}(y) - \nabla^2 \mathcal{L}(x)} \leq Mr
%         $$        
%     \end{proof}

%     In particular, the constant $r$ is necessary, especially since hyper-parameters can potentially modify data (for example, consider a hyper-parameter that chooses between different data preprocessing methods). If the hyper-parameter space is restricted so that the data is guaranteed to be the same (i.e., the hyper-parameters affect the loss landscape without the underlying data), then we can guarantee a better bound:
%     \begin{lemma}[Smoothness approximation bound in restricted case]
%         Consider the restricted formulation above. The maximum approximation error is given by $\beta_{max}$.
%     \end{lemma}
%     \begin{proof}
%         Because $\mathcal{L}$ is $\beta-$smooth with varying values of $\beta$, we have $\norm{\nabla^2 \mathcal{L}} \leq \beta_{max}$. By definition of a norm, $\norm{\nabla^2 \mathcal{L}} \geq 0$, so that $\beta_{max} - \mu_{min} \leq \beta_{max}$. In particular, this occurs when $\mu_{min} = 0$ (i.e., for that choice of hyper-parameters, the function is not strongly convex).
%     \end{proof}
    
%     \item  \textit{Maximizing smoothness yields flatter loss surfaces.}
%     Empirically, we observed that the loss surfaces obtained by maximizing smoothness had flat minima. For example, Figure \ref{fig:smoothness-hpo} shows the resulting loss landscape for the MNIST dataset. This is known to have consequences for generalization performance. See Section \ref{sec:background} for work on flat minima.
% \end{enumerate}
